Emergence of Order in Dynamical Phases in Coupled Fractional Gauss Map

Dynamical behaviour of discrete dynamical systems has been investigated extensively in the past few decades. However, in several applications, long term memory plays an important role in the evolution of dynamical variables. The definition of discrete maps has recently been extended to fractional maps to model such situations. We extend this definition to a spatiotemporal system. We define a coupled map lattice on different topologies, namely, one-dimensional coupled map lattice, globally coupled system and small-world network. The spatiotemporal patterns in the fractional system are more ordered. In particular, synchronization is observed over a large parameter region. For integer order coupled map lattice in one dimension, synchronized periodic states with a period greater than one are not obtained. However, we observe synchronized periodic states with period-3 or period-6 in one dimensional coupled fractional maps even for a large lattice. With nonlocal coupling, the synchronization is reached over a larger parameter regime. In all these cases, the standard deviation decays as power-law in time with the power same as fractional-order. The physical significance of such studies is also discussed.

==> biblio <==
Deshpande, A. and Daftardar-Gejji, V., 2016. Chaos in discrete fractional difference equations. Pramana, 87(4), p.49.
\bibitem{atici2009initial}
Atici, F. and Eloe, P., 2009. Initial value problems in discrete fractional calculus. Proceedings of the American Mathematical Society, 137(3), pp.981-989.
\bibitem{socolar1994stabilizing}
Socolar, J.E., Sukow, D.W. and Gauthier, D.J., 1994. Stabilizing unstable periodic orbits in fast dynamical systems. Physical Review E, 50(4), p.3245.
\bibitem{gomez2018fundamental}
Gómez-Aguilar, J.F., 2018. Fundamental solutions to electrical circuits of non-integer order via fractional derivatives with and without singular kernels. The European Physical Journal Plus, 133(5), p.197.
\bibitem{yang2018advanced}
Yang, X.J., Baleanu, D. and Srivastava, H.M., 2018. Advanced analysis of local fractional calculus applied to the Rice theory in fractal fracture mechanics.
\bibitem{metzler2003fractional}
Metzler, R. and Nonnenmacher, T.F., 2003. Fractional relaxation processes and fractional rheological models for the description of a class of viscoelastic materials. International Journal of Plasticity, 19(7), pp.941-959.
\bibitem{tarasov2011fractional}
Tarasov, V.E., 2011. Fractional dynamics: applications of fractional calculus to dynamics of particles, fields and media. Springer Science \& Business Media.
\bibitem{podlubny1998fractional}
Podlubny, I., 1998. Fractional differential equations: an introduction to fractional derivatives, fractional differential equations, to methods of their solution and some of their applications (Vol. 198). Elsevier.
\bibitem{sheng2011fractional}
Sheng, H., Chen, Y. and Qiu, T., 2011. Fractional processes and fractional-order signal processing: techniques and applications. Springer Science \& Business Media.
\bibitem{wu2014discrete}
Wu, G.C. and Baleanu, D., 2014. Discrete fractional logistic map and its chaos. Nonlinear Dynamics, 75(1-2), pp.283-287.
\bibitem{oldham1974fractional}
Oldham, K. and Spanier, J., 1974. The fractional calculus theory and applications of differentiation and integration to arbitrary order (Vol. 111). Elsevier.
\bibitem{samko1993fractional}
Samko, S.G., Kilbas, A.A. and Marichev, O.I., 1993. Fractional integrals and derivatives: theory and applications.
\bibitem{magin2006fractional}
Magin, R.L., 2006. Fractional calculus in bioengineering (pp. 269-355). Redding: Begell House.
\bibitem{daftardar2013fractional}
Daftardar-Gejji, V.,editor, 2013. Fractional calculus: Theory and applications. Narosa, New Delhi.
\bibitem{atici2010modeling}
Atıcı, F.M. and Şengül, S., 2010. Modeling with fractional difference equations. Journal of Mathematical Analysis and Applications, 369(1), pp.1-9.
\bibitem{rudolf2000applications}
Rudolf, H. ed., 2000. Applications of fractional calculus in physics. World Scientific.
\bibitem{kilbas2006theory}
Kilbas, A.A.A., Srivastava, H.M. and Trujillo, J.J., 2006. Theory and applications of fractional differential equations (Vol. 204). Elsevier Science Limited.
\bibitem{lakshmikantham2009theory}
Lakshmikantham, V., Leela, S. and Devi, J.V., 2009. Theory of fractional dynamic systems. CSP.
\bibitem{diethelm2002analysis}
Diethelm, K. and Ford, N.J., 2002. Analysis of fractional differential equations. Journal of Mathematical Analysis and Applications, 265(2), pp.229-248.
\bibitem{metzler2000random}
Metzler, R. and Klafter, J., 2000. The random walk's guide to anomalous diffusion: a fractional dynamics approach. Physics reports, 339(1), pp.1-77.
\bibitem{mainardi2010fractional}
Mainardi, F., 2010. Fractional calculus and waves in linear viscoelasticity: an introduction to mathematical models. World Scientific.

